Convergence of Edge Computing and Deep Learning: A Comprehensive Survey

Ubiquitous sensors and smart devices from factories and communities are generating massive amounts of data, and ever-increasing computing power is driving the core of computation and services from the cloud to the edge of the network. As an important enabler broadly changing people's lives, from face recognition to ambitious smart factories and cities, developments of artificial intelligence (especially deep learning, DL) based applications and services are thriving. However, due to efficiency and latency issues, the current cloud computing service architecture hinders the vision of "providing artificial intelligence for every person and every organization at everywhere". Thus, unleashing DL services using resources at the network edge near the data sources has emerged as a desirable solution. Therefore, edge intelligence, aiming to facilitate the deployment of DL services by edge computing, has received significant attention. In addition, DL, as the representative technique of artificial intelligence, can be integrated into edge computing frameworks to build intelligent edge for dynamic, adaptive edge maintenance and management. With regard to mutually beneficial edge intelligence and intelligent edge, this paper introduces and discusses: 1) the application scenarios of both; 2) the practical implementation methods and enabling technologies, namely DL training and inference in the customized edge computing framework; 3) challenges and future trends of more pervasive and fine-grained intelligence. We believe that by consolidating information scattered across the communication, networking, and DL areas, this survey can help readers to understand the connections between enabling technologies while promoting further discussions on the fusion of edge intelligence and intelligent edge, i.e., Edge DL.

==> Fundamentals.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Fundamentals of Deep Learning and Edge Computing}
\label{sec:fundamentals}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With respect to the community of Computer Vision (CV), Natural Language Processing (NLP), and Artificial Intelligence (AI), Deep Learning (DL) is adopted in a myriad of applications and corroborates its superior performance \cite{placeholder}. On the other hand, aiming for seamlessly bringing in Edge Computing (EC) to push computing resources away from the centralized cloud, the evolution of the communication and network architecture is looming. In this section, we only compendiously provide concepts of deep learning and edge computing, and define technical terms for following sections, without describing their combination.

\subsection{Neural Network in Deep Learning}
\label{subsec:nndl}

The ``deep'' in DL means that only Neural Networks (NNs) with a sufficient number of NN layers can be deemed as Deep Neural Networks (DNNs)\cite{haykin2009neural}. Such kind of DL models consist of various types of NNs. In Fig. \ref{fig1:NeuralNetwork}, we directly introduce the fundamental type of NNs in DL, focusing on the basic structure and function of them (details of high quality can be find in \cite{placeholder}).

\subsubsection{Fully Connected Neural Network}
\label{subsubsec:fcnn}

Fully Connected Neural Network (FCNN) layer \cite{Collobert:2004:LPM:1015330.1015415}, as in Fig. \ref{fig1:NeuralNetwork}(a), is the initial design of Artificial Neutral Network (ANN), and constitutes the FCNN, i.e., Multilayer Perceptron (MLP). The output of each layer of FCNN is fed forward to the next layer in a feedforward fashion. Between contiguous FCNN layers, the output of a neuron is directly passed to neurons belong to the next layer, noticing that there are no convolutional or recurrent computation except activation function. In virtue of the deep version of this simple structure, FCNN can be used for feature extraction and function approximation, however, with high complexity, modest performance and slow convergence.

\subsubsection{Autoencoder}
\label{subsubsec:autoencoder}

Autoencoder includes two processes of encode and decode. We usually choose the neural network model as the encoder and decoder. At runtime, the input training samples are first dimension reduced by the encoder. Then the processed sample is input to the decoder to obtain a generated data. Finally, compare the difference between the original training samples and the generated data, and train the parameters of the encoder and decoder by narrowing the difference.

\subsubsection{Convolutional Neural Network}
\label{subsubsec:cnn}

Convolutional Neural Network (CNNs), shown in Fig. \ref{fig1:NeuralNetwork}(b), are a common form of DNNs. By employing a set of distinct moving filters, CNNs seize correlations between adjacent data pieces, and then generate a successively higher level abstraction of the input data \cite{10.1007/978-3-319-10590-1_53}. Compared to FCNNs, CNNs extract the features while reducing the model complexity, which mitigates the risk of overfitting. These characteristics make CNNs achieve remarkable performance in image processing and also useful in processing structural data similar to images.

\subsubsection{Recurrent Neural Network}
\label{subsubsec:rnn}

Recurrent Neural Networks (RNNs) are feedforward neural networks that consider handling sequential data in time domain \cite{Schmidhuber2015}. As depicted in Fig. \ref{fig1:NeuralNetwork}(c), the neuron in RNNs not only receives information from the upper layer of the neural network, but also receives information from the previous channel. In general, RNNs are a good choice for predicting future information or complementing information such as applications in NLP. The biggest problem with recurrent neural networks is that the gradient disappears (or gradient explosion).

Long Short-Term Memory (LSTM) \cite{Hochreiter:1997:LSM:1246443.1246450} is designed to overcome these problems by introducing a gate structure and a well-defined memory cell. Each neuron has a memory unit and three gate structures: input, output, and forget. The function of these gate structures is to protect information by prohibiting or allowing the flow of information. The input gate structure determines how much information from the previous layer is stored in the current memory unit. The output gate structure takes over the work at the other end and determines how much of this layer of information can be learned by the next layer.

\subsubsection{Generative Adversarial Network}
\label{subsubsec:gan}

Generative Adversarial Network (GAN) originates from the Nash equilibrium of game theory. As showned in Fig \ref{fig1:NeuralNetwork}(d), GAN is composed of generator and discriminator. The goal of the generator is to learn as much as possible about the true data distribution, while the discriminator is to determine correctly whether the input data is coming from the true data or the generator. In order to win the game, these two participants need to constantly optimize their ability to generate and distinguish in the adversarial process. This optimize process is to find a Nash equilibrium between them.

\subsection{Deep Reinforcement Learning}

Traditional reinforcement learning is limited to the small action space and sample space. When the input data is images and sounds, it often has a high dimension, which is difficult to deal with by reinforcement learning. Fortunately, Deep reinforcement learning (DRL) combines the high dimensional input of deep learning with reinforcement learning, which can solve this problem. Nowadays, DRL has become a powerful method and made remarkable progress in robotics, natural language processing, computer vision, neural architecture design, business management, finance, healthcare and other fields\cite{Mousavi2018}.

\subsubsection{Markov Decision Process}

The Markov decision process is an optimal decision process for a stochastic dynamic system. In this process, the decision maker can periodically observe the stochastic dynamic system with Markov property, and select an action from the set of available actions to make decisions according to the state observed at each moment.

In reinforcement learning, agents and environments have been interacting with each other. The Agent can receive the status of the current environment and generate actions based on it, and then act on the environment. After that, it returns a revenue value according to the effect of the action, so that the agent updates. Therefore, a sequence is formed during the constant interaction between the agent and the environment, and this process is a sequence decision process. The Markov decision process is the formulation of this process and provides a convenient and practical means.


\subsubsection{Value-based DRL}

As a representative of Value-based DRL, Deep $Q$-Learning (DQL) was proposed by DeepMind \cite{Mnih2015}, which has many improvements compared to previous methods. First, it uses a convolutional neural network to fit action values in reinforcement learning, successfully filling the gap between high-dimensional input data and action. Secondly, in order to ensure stable convergence of training, experience replay method is adopted to break the correlation between data collected. Finally, since the previous training methods often have numerical instability, the DQL sets up a separate target network, updating its parameters every fixed number of steps.However, DQN still has many shortcomings. In order to solve these problems, DQN has derived many improved versions.

After DQN was proposed, researchers found and proved that DQN generally overestimates the action values, and the estimated error increases with the number of actions\cite{Hasselt2015Deep}. In response to this problem, they proposed the Double Deep $Q$-Learning (DDQL). The specific measure taken is to use the different values to select and evaluate the actions. Whenever parameters are updated, one of the value function is used for action selection, and another function is used to evaluate action values.

In addition, some researchers have proposed another improvement to DQL, Dueling Deep $Q$-Learning \cite{Wang2015Dueling}. Its main idea is to divide the value function into the state value function and the state-dependent action advantage function, and finally calculate the action values by adding them together. Therefore, the value of a state can be learned without being affected by the actions of this state. Experiments have also shown that when similar actions are added, the model can quickly learn the value of these new actions without having to relearn the value of the state.

More interestingly, some researchers have tried to combine some of DQN's improved versions and have achieved good results through experimental verification\cite{Hessel2017}.

\subsubsection{Policy-gradient-based DRL}

There is another type called Policy-gradient-based DRL, which no longer calculates action values, but directly makes decisions based on the input of the state. The Actor-Critic algorithm is a combination of the two, which mainly includes actor and critic. The Actor is similar to the Policy-gradient-based DRL, which inputs the state, outputs the actions through the neural network and selects the appropriate action from a certain probability in these continuous actions. But the critic similar to Value-based DRL which feeds back to the actor by calculating the value, helping the actor to make policy adjustments. However, the convergence of the Actor-Critic algorithm is not good, so many improved versions have also been proposed.

Mnih et al. proposed the Asynchronous Advantage Actor-Critic (A3C) method\cite{pmlr-v48-mniha16}. To train a pair of actor and critic, they copy actor and critic into multiple copies, then put them in different environments. After that, the parameters in the main agent are updated by these copies. Since the copies in the parallel do not interfere with each other, the correlation of the update is reduced and the convergence is improved.

As another improvement of Actor-Critic, deepmind proposed the Deep Deterministic Policy Gradient (DDPG) method\cite{lillicrap2015continuous}. This approach introduces the idea of DQN into Actor-Critic. It adds experience replay and a separate target network to the actor and critic, which improves the convergence of the training.

Proximate policy optimization (PPO) is also an excellent method in Policy-gradient-based DRL \cite{Schulman2017Proximal}. Because the step size during training is usually difficult to determine. If the setting is too large, the training will be difficult to converge. If the setting is too small, the training time will be too long. They propose a novel objective function that enables small batch updates in multiple training steps.

In addition, when dealing with large discrete action spaces, Dulac-Arnold et al. introduced the idea of action embedding by embedding discrete actions into small spaces, which allows the use of traditional DRL methods\cite{Dulac-arnold}.


\subsection{Distributed Training}

At present, the training of the model consumes a lot of time and computing resources, which becomes the main bottleneck for further improving the performance of the algorithm. Therefore, adopting a distributed training method is a good choice. On the one hand, this can speed up the training and reduce the response time. On the other hand, the model can use more training samples during training to improve the accuracy of the model.

There are two common ways to parallelize training. One is by creating multiple copies of the model with the same structure and having each copy train a portion of the data samples in parallel, which is called data parallelism. Another way is to split the large model structure into multiple parts to run in parallel, which is called model parallelism. At present, some related platforms are already available. For example, the DistBelief framework proposed by Jeffrey Dean et al. supports both data parallelism and model parallelism\cite{Monin1981}. Tencent built Mariana uses GPU and CPU clusters for parallel training, supports multi-GPU data parallel framework for deep neural networks, and deep convolutional neural networks. GPU model parallel and data parallel framework, and CPU cluster framework for deep neural networks\cite{zou2014mariana}.

\subsubsection{Training Principles}

When using the sample data to train the model, the model will constantly adjust the parameters to bring the predicted values closer to the actual values. For this purpose, a function is usually defined to describe the difference between the predicted value and the actual value, called loss function. Thus, the training of the model can be transformed into a problem that minimizes the loss function. To solve this problem, a gradient descent method is usually used, that is, for a given parameter and loss function, the algorithm minimizes the loss function by updating the parameters in the opposite direction of the gradient. For example, Stochastic Gradient Descent (SGD) is a representative of this kind of method, which first assigns a set of initial values to the parameters, and then randomly selects a data from the training sample set and updates the parameters with it in each iteration, and finally ends when the convergence state is reached.

\subsubsection{Model Parallelism}

Model parallelism is run in parallel by splitting large models into multiple parts. This not only can improve the training speed, but also solves the problem that the model is larger than device memory. Training a large model often requires a lot of computing resources. Therefore, researchers often use thousands of CPUs to train a model. In order to solve this problem, the COTS HPC system proposed by A. Coates et al. can use the GPU for model parallel training. They use three GPU servers to complete the deep neural network training of 1 billion parameters in a few days\cite{Ltifi2010}. In addition, Xie Chen et al. also proposed a multi-GPGPU parallel training approach and applied the idea of pipelined back-propagation\cite{Chen2012}.

\subsubsection{Data Parallelism}

Data parallelism is the process of dividing data into multiple parts and using multiple copies of the model to parallel training. This can reduce the time of model training and improve training efficiency. Currently, widely-popular frameworks such as spark have already supported this method \cite{Nishihara2016}. Today, many global services run on data centers distributed around the world. Although there are high-bandwidth networks within the data center, the quality of the network between the data centers is poor, which can affect the training of the model. To deal with this challenge, the author of \cite{Hsieh2017} proposes the approximate synchronous parallel model to reduce communication between data centers and improve performance. In \cite{Wen2017}, the authors observed that when parameters such as gradient were transmitted, a large network burden would be generated, so they proposed TernGrad to quantify the gradient into three values, thus further reducing the communication. In addition, \cite{Iandola} proposed that the traffic could be reduced by using high bandwidth network hardware, using the communication algorithm of reduction trees and increasing the batch size.

\subsection{Transfer Learning}

Transfer Learning (TL) is a machine learning method that transfers knowledge from source domain to target domain so as to achieve better learning results in the target domain. By using transfer learning, you can reuse existing knowledge and reduce the huge development costs of new areas. However, there is a problem with transfer learning. It is often applied to some small and stable data sets, making it difficult to get a wider application.

Similarly, Knowledge Distillation (KD) is also a way to solve problems by reusing knowledge. It was first proposed by Hinton et al. \cite{hinton2015distilling }, which introduced the training of the student network by introducing a soft-targe associated with the teacher network as part of the total loss. In addition, experiments have shown that by compressing a deep network into a shallow network, it can still mimic the functions of deep networks \cite{ba2014deep}, which provides a powerful help for its wide application.


\subsection{Mainstream Deep Learning Libraries}

As the heat of deep learning continues to rise, various deep learning libraries are also emerging, which provides a convenient way for the application and research of deep learning. In this section, we have selected several types of mainstream deep learning libraries for a brief introduction.

\subsubsection{TensorFlow}

TensorFlow is a very popular deep learning library \cite{Abadi2016}. On the one hand, it can help users to easily build a neural network, on the other hand it has a TensorBoard component that can monitor the running process and visualize the computation graph. The core code of TensorFlow is written in C++, which greatly improves the efficiency of the model deployment. In addition, it also implements interfaces such as Python, Go, and Java through Simplified Wrapper and Interface Generator (SWIG), which provides excellent support for different kinds of models.

\subsubsection{Caffe}

The core concept of Convolutional Architecture for Fast Feature Embedding (Caffe) is layer, which can input data and perform calculations internally to output the results \cite{jia2014caffe}. Multiple layers can be stitched together to form a complete neural network. Caffe has a large number of trained models stored in the Model Zoo, so it is very convenient to use. In addition, the underlying Caffe is based on C++ and is easy to deploy in different environments. It is widely used in computer vision such as face recognition \cite{wen2016discriminative}, image classification \cite{yu2017convolutional}, and target tracking \cite{hong2015online}.

\subsubsection{Theano}

At the heart of Theano is a mathematical expression compiler for large-scale neural network training that compiles user-designed calculations into machine code execution \cite{bergstra2010theano}. Theano is a deep learning library based on Python, so the deployment of the model is very inconvenient and the application on mobile devices is lacking. In addition, Theano has derived many deep learning libraries, such as Keras, Lasagne and so on.

\subsubsection{PyTorch}

PyTorch is a deep learning library derived from Torch. Since PyTorch supports the creation of a dynamic computation graph, it constructs a graph for each line of code as part of a complete computational graph. Even if the complete calculation diagram is not yet built, we can perform these small calculation diagrams as components independently, so it has flexible process control capabilities. In addition, compared to many deep learning libraries that need to record a tape to record the order of operations, PyTorch uses the reverse-mode automatic differentiation method to cancel the tape \cite{paszke2017automatic}.

\subsubsection{MXNET}

MXNet is a lightweight deep learning library \cite{Chenb}. MXNet is one of the earliest supported distributed computing in various deep learning libraries. It supports automatic parallelization of computing tasks to multiple GPUs or distributed clusters, and has good distributed performance. Another advantage of MXNet is that it consumes less hardware resources. MXNet is a good choice for many models that cannot be trained due to insufficient hardware resources in other deep learning libraries.

\subsection{Edge Computing}

Edge Computing Nowadays, with the popularity of mobile devices, various types of network applications are emerging one after another, such as multimedia applications, VR online games and other applications attract a lot of attention \cite{jung2011cisco}. The generation of these applications also gives the current network a higher requirement in terms of delay, bandwidth and other indicators.

Edge computing technology is expected to solve this problem fundamentally. It reduces data transmission distance and optimizes bandwidth by migrating part of the computational load closer to the edge of the data source. This will bring many benefits. On the one hand, processing part of the computing task on the edge side can reduce the bandwidth pressure in the network. On the other hand, it responds to the task on the edge side, reducing the transmission delay and improving the response speed.

\subsubsection{End Devices}

There are a variety of end devices for edge computing, such as smart phones, virtual reality glasses, smart cameras and so on. They are producers of data and tasks, with functions of data preprocessing and data transmission. The computing resources required by these devices are usually huge, and it is difficult to meet the needs by relying on the computing capability of the devices themselves. Therefore, it can be solved by edge computing with the help of computing resources at the edge end and in the cloud.

\subsubsection{Edge Nodes}

Edge node is close to the end devices. It has computing and caching capabilities and can provide high-quality network connection and computing services for the end devices. Compared with end devices, edge nodes have more powerful computing capability to process tasks. Compared with the cloud, edge nodes have faster response speed to end devices. Therefore, by using edge nodes to perform some computing tasks, the response speed of tasks can be improved while ensuring accuracy. In addition, edge nodes also have the ability to cache, which can improve the response time on re-visit by saving the object with a large number of visits to the cache device.

\subsubsection{Edge Devices}


\subsubsection{Relation with Cloud Computing}

Cloud computing is a centralized data processing method. It first transmits data to the cloud by the end device, and then processes the data through the cloud to return the result to the end device. Cloud computing has good support for computationally intensive tasks, but with the explosive growth of data generated by end devices, cloud computing faces many challenges. On the one hand, cloud computing needs to transfer a large amount of data to the cloud, which will inevitably cause extremely high transmission delay and reduce the response speed to the task. On the other hand, a large amount of data needs to rely on the network for transmission, which will bring heavy pressure on the network. In addition, privacy, energy consumption and other problems caused by massive data transmission are also difficult to solve. Therefore, in order to solve these challenges, edge computing came into being. Compared to cloud computing, edge computing sets edge nodes with computation and caching capabilities close to the location of the end device. Therefore, some data need not be transferred to the cloud, but to the edge node close to the end device for processing, so as to reduce the transmission delay and network cost caused by data going to and from the cloud.





==> Tables/TableAbbreviationsV1.tex <==
% \begin{table}[tp]  
%     \centering  
%     \begin{threeparttable}  
%         \caption{List of abbreviations in alphabetical order.}  
%         \label{tab:abbreviation}  
%         \begin{tabular}{cl}  
%             \toprule  
%             \multicolumn{1}{c}{\bf Abbreviation}&\multicolumn{1}{c}{\bf Description}\cr
%             \midrule  
             
%             AC&Actor-Critic\cr
%             A3C&Asynchronous Advantage Actor-Critic\cr
%             AE&Auto-Encoder\cr
%             AI&Artificial Intelligence\cr
%             APU&AI Processing Unit\cr
%             AR&Augmented Reality\cr
%             ASIC&Application-Specific Integrated Circuit\cr
% %B
%             BER&Bit Error Rate\cr
% %C
%             C-RAN&Cloud-Radio Access Networks\cr
%             CDN&Content Delivery Network\cr
%             CNN&Convolutional Neural Network\cr
%             CV&Computer Vision\cr
% %D
%             D2D&Device-to-Device\cr
%             DDoS&Distributed Denial of Service\cr
%             DDPG&Deep Deterministic Policy Gradien\cr
%             DGC&Deep Gradient Compression\cr
%             DL&Deep Learning\cr
%             DNNs&Deep Neural Networks\cr
%             Double-DQL&Double Deep $Q$-Learning\cr
%             DQL&Deep $Q$-Learning\cr
%             DRAM&Dynamic RAM\cr
%             DRL&Deep Reinforcement Learning\cr
%             Dueling-DQL&Dueling Deep $Q$-Learning\cr
%             DVFS&Dynamic Voltage and Frequency Scaling\cr
% %E
%             ECSP&Edge Computing Service Provider\cr
%             EEoI&Early Exit of Inference\cr
%             EH&Energy Harvesting\cr
%             ETSI&European Telecommunications Standards Institute\cr
% %F
%             FAP&Fog radio Access Point\cr
%             FCNN&Fully Connected Neural Network\cr
%             FL&Federated Learning\cr
%             FPGA&Field Programmable Gate Array\cr
%             FTP&Fused Tile Partitioning\cr
% %G
%             GAN&Generative Adversarial Network\cr
%             GNNs&Graph Neural Networks\cr
% %H
% %I
%             IID&Independent and Identically Distributed\cr
%             IoT&Internet of Things\cr
%             IoVs&Internet of Vehicles\cr
% %J
% %K
%             KD&Knowledge Distillation\cr
%             KNN&K-Nearest Neighbor\cr
% %L
% %M
%             MAB&Multi-Armed Bandit\cr
%             MDCs&Micro Data Centers\cr
%             MDP&Markov Decision Process\cr
%             MLP&Multi-Layer Perceptron\cr
%             % MSNs&Mobile Social Networks\cr
% %N
%             NLP&Natural Language Processing\cr
%             NNs&Neural Networks\cr
%             NPU&Neural Processing Unit\cr
% %O
% %P
%             PPO&Proximate Policy Optimization\cr
% %Q
% %R
%             RNN&Recurrent Neural Network\cr
%             RoIs&Region-Of-Interest\cr
%             RRH&Remote Radio Head\cr
%             RSU&Road-Side Units\cr
% %S
%             SDN&Software-Defined Network\cr
%             SINR&Signal-to-Interference-plus-Noise Ratio\cr
%             SNPE&Snapdragon Neural Processing Engine\cr
%             % SNR&Signal-to-Noise Rations\cr
%             SRAM&Static Random Access Memory\cr
% %T
%             TL&Transfer Learning\cr
% %U
%             URLLC& Ultra-Reliable Low-Latency Communications\cr
% %V
%             VM&Virtual Machine\cr
%             VR&Virtual Reality\cr
%             V2V&Vehicle-to-Vehicle\cr
% %W          
%             WLAN&Wireless Local Area Network\cr
% %X
% %Y
% %Z
%             ZB&Zettabytes\cr
                            
%             \bottomrule  
%         \end{tabular}  
%     \end{threeparttable}  
% \end{table}


% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%     \centering
%     \scriptsize
%     \caption{List of Abbreviations in Alphabetical Order}
%       \begin{tabular}{clcl}
%       \toprule
%       Abbr. & \multicolumn{1}{c}{Definition} & Abbr. & \multicolumn{1}{c}{Definition} \\
%       \midrule
%       AC    & Actor-Critic & FTP   & Fused Tile Partitioning \\
%       \midrule
%       A3C   & Asynchronous Advantage Actor-Critic & GAN   & Generative Adversarial Network \\
%       \midrule
%       AE    & Auto-Encoder & GNNs  & Graph Neural Networks \\
%       \midrule
%       AI    & Artificial Intelligence & IID   & Independent and Identically Distributed \\
%       \midrule
%       APU   & AI Processing Unit & IoT   & Internet of Things \\
%       \midrule
%       AR    & Augmented Reality & IoVs  & Internet of Vehicles \\
%       \midrule
%       ASIC  & Application-Specific Integrated Circuit & KD    & Knowledge Distillation \\
%       \midrule
%       BER   & Bit Error Rate & KNN   & K-Nearest Neighbor \\
%       \midrule
%       BS    & Base Station & MAB   & Multi-Armed Bandit \\
%       \midrule
%       C-RAN & Cloud-Radio Access Networks & MDCs  & Micro Data Centers \\
%       \midrule
%       CDN   & Content Delivery Network & MDP   & Markov Decision Process \\
%       \midrule
%       CNN   & Convolution Neural Network & MLP   & Multi-Layer Perceptron \\
%       \midrule
%       CV    & Computer Vision & NLP   & Natural Language Processing \\
%       \midrule
%       D2D   & Device-to-Device & NN    & Neural Network \\
%       \midrule
%       DDoS  & Distributed Denial of Service & NPU   & Neural Processing Unit \\
%       \midrule
%       DDPG  & Deep Deterministic Policy Gradient & PPO   & Proximate Policy Optimization \\
%       \midrule
%       DGC   & Deep Gradient Compression & RNN   & Recurrent Neural Network \\
%       \midrule
%       DL    & Deep Learning & RoI   & Region-of-Interest \\
%       \midrule
%       DNNs  & Deep Neural Networks & RRH   & Remote Radio Head \\
%       \midrule
%       DQL   & Deep Q-Learning & RSU   & Road-Side Unit \\
%       \midrule
%       DRAM  & Dynamic RAM & SDN   & Software-Defined Network \\
%       \midrule
%       DRL   & Deep Reinforcement Learning & SINR  & Signal-to-Interference-plus-Noise Ratio \\
%       \midrule
%       DVFS  & Dynamic Voltage and Frequency Scaling & SNPE  & Snapdragon Neural Processing Engine \\
%       \midrule
%       ECSP  & Edge Computing Service Provider & SRAM  & Static Random Access Memory \\
%       \midrule
%       EEoI  & Early Exit of Inference & TL    & Transfer Learning \\
%       \midrule
%       EH    & Energy Harvesting & URLLC & Ultra-Reliable Low-Latency Communications \\
%       \midrule
%       ETSI  & European Telecommunications Standards Institute & VM    & Virtual Machine \\
%       \midrule
%       FAP   & Fog radio Access Point & VR    & Virtual Reality \\
%       \midrule
%       FCNN  & Fully Connected Neural Network & V2V   & Vehicle-to-Vehicle \\
%       \midrule
%       FL    & Federated Learning & WLAN  & Wireless Local Area Network \\
%       \midrule
%       FPGA  & Field Programmable Gate Array & ZB    & Zettabytes \\
%       \bottomrule
%       \end{tabular}%
%     \label{tab:abbreviation}%
%   \end{table*}%
  
  
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \scriptsize
%   \caption{List of Abbreviations in Alphabetical Order}
%     \begin{tabular}{clclrr}
%     \toprule
%     Abbr. & \multicolumn{1}{c}{Definition} & Abbr. & \multicolumn{1}{c}{Definition} & \multicolumn{1}{c}{Abbr.} & \multicolumn{1}{c}{Definition} \\
%     \midrule
%     AC    & Actor-Critic & DRL   & Deep Reinforcement Learning & \multicolumn{1}{c}{MLP} & \multicolumn{1}{l}{Multi-Layer Perceptron} \\
%     \midrule
%     A3C   & Asynchronous Advantage Actor-Critic & DVFS  & Dynamic Voltage and Frequency Scaling & \multicolumn{1}{c}{NLP} & \multicolumn{1}{l}{Natural Language Processing} \\
%     \midrule
%     AE    & Auto-Encoder & ECSP  & Edge Computing Service Provider & \multicolumn{1}{c}{NN} & \multicolumn{1}{l}{Neural Network} \\
%     \midrule
%     AI    & Artificial Intelligence & EEoI  & Early Exit of Inference & \multicolumn{1}{c}{NPU} & \multicolumn{1}{l}{Neural Processing Unit} \\
%     \midrule
%     APU   & AI Processing Unit & EH    & Energy Harvesting & \multicolumn{1}{c}{PPO} & \multicolumn{1}{l}{Proximate Policy Optimization} \\
%     \midrule
%     AR    & Augmented Reality & ETSI  & European Telecommunications Standards Institute & \multicolumn{1}{c}{RNN} & \multicolumn{1}{l}{Recurrent Neural Network} \\
%     \midrule
%     ASIC  & Application-Specific Integrated Circuit & FAP   & Fog radio Access Point & \multicolumn{1}{c}{RoI} & \multicolumn{1}{l}{Region-of-Interest} \\
%     \midrule
%     BER   & Bit Error Rate & FCNN  & Fully Connected Neural Network & \multicolumn{1}{c}{RRH} & \multicolumn{1}{l}{Remote Radio Head} \\
%     \midrule
%     BS    & Base Station & FL    & Federated Learning & \multicolumn{1}{c}{RSU} & \multicolumn{1}{l}{Road-Side Unit} \\
%     \midrule
%     C-RAN & Cloud-Radio Access Networks & FPGA  & Field Programmable Gate Array & \multicolumn{1}{c}{SDN} & \multicolumn{1}{l}{Software-Defined Network} \\
%     \midrule
%     CDN   & Content Delivery Network & FTP   & Fused Tile Partitioning & \multicolumn{1}{c}{SGD} & \multicolumn{1}{l}{Stochastic Gradient Descent} \\
%     \midrule
%     CNN   & Convolutional Neural Network & GAN   & Generative Adversarial Network & \multicolumn{1}{c}{SINR} & \multicolumn{1}{l}{Signal-to-Interference-plus-Noise Ratio} \\
%     \midrule
%     CV    & Computer Vision & GNNs  & Graph Neural Networks & \multicolumn{1}{c}{SNPE} & \multicolumn{1}{l}{Snapdragon Neural Processing Engine} \\
%     \midrule
%     D2D   & Device-to-Device & IID   & Independent and Identically Distributed & \multicolumn{1}{c}{SRAM} & \multicolumn{1}{l}{Static Random Access Memory} \\
%     \midrule
%     DDoS  & Distributed Denial of Service & IoT   & Internet of Things & \multicolumn{1}{c}{TL} & \multicolumn{1}{l}{Transfer Learning} \\
%     \midrule
%     DDPG  & Deep Deterministic Policy Gradient & IoVs  & Internet of Vehicles & \multicolumn{1}{c}{VM} & \multicolumn{1}{l}{Virtual Machine} \\
%     \midrule
%     DGC   & Deep Gradient Compression & KD    & Knowledge Distillation & \multicolumn{1}{c}{VR} & \multicolumn{1}{l}{Virtual Reality} \\
%     \midrule
%     DL    & Deep Learning & KNN   & K-Nearest Neighbor & \multicolumn{1}{c}{V2V} & \multicolumn{1}{l}{Vehicle-to-Vehicle} \\
%     \midrule
%     DNNs  & Deep Neural Networks & MAB   & Multi-Armed Bandit & \multicolumn{1}{c}{WLAN} & \multicolumn{1}{l}{Wireless Local Area Network} \\
%     \midrule
%     DQL   & Deep Q-Learning & MDCs  & Micro Data Centers & \multicolumn{1}{c}{ZB} & \multicolumn{1}{l}{Zettabytes} \\
%     \midrule
%     DRAM  & Dynamic RAM & MDP   & Markov Decision Process &       &  \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:abbreviation}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \scriptsize
  \caption{List of Abbreviations in Alphabetical Order}
    \begin{tabular}{clclrr}
    \toprule
    Abbr. & \multicolumn{1}{c}{Definition} & Abbr. & \multicolumn{1}{c}{Definition} & \multicolumn{1}{c}{Abbr.} & \multicolumn{1}{c}{Definition} \\
    \midrule
    AC    & Actor-Critic & DVFS  & Dynamic Voltage and Frequency Scaling & \multicolumn{1}{c}{NN} & \multicolumn{1}{l}{Neural Network} \\
    \midrule
    A3C   & Asynchronous Advantage Actor-Critic & ECSP  & Edge Computing Service Provider & \multicolumn{1}{c}{NPU} & \multicolumn{1}{l}{Neural Processing Unit} \\
    \midrule
    AE    & Auto-Encoder & EEoI  & Early Exit of Inference & \multicolumn{1}{c}{PPO} & \multicolumn{1}{l}{Proximate Policy Optimization} \\
    \midrule
    AI    & Artificial Intelligence & EH    & Energy Harvesting & \multicolumn{1}{c}{QoE} & \multicolumn{1}{l}{Quality of Experience} \\
    \midrule
    APU   & AI Processing Unit & ETSI  & European Telecommunications Standards Institute & \multicolumn{1}{c}{QoS} & \multicolumn{1}{l}{Quality of Service} \\
    \midrule
    AR    & Augmented Reality & FAP   & Fog radio Access Point & \multicolumn{1}{c}{RNN} & \multicolumn{1}{l}{Recurrent Neural Network} \\
    \midrule
    ASIC  & Application-Specific Integrated Circuit & FCNN  & Fully Connected Neural Network & \multicolumn{1}{c}{RoI} & \multicolumn{1}{l}{Region-of-Interest} \\
    \midrule
    BER   & Bit Error Rate & FL    & Federated Learning & \multicolumn{1}{c}{RRH} & \multicolumn{1}{l}{Remote Radio Head} \\
    \midrule
    BS    & Base Station & FPGA  & Field Programmable Gate Array & \multicolumn{1}{c}{RSU} & \multicolumn{1}{l}{Road-Side Unit} \\
    \midrule
    C-RAN & Cloud-Radio Access Networks & FTP   & Fused Tile Partitioning & \multicolumn{1}{c}{SDN} & \multicolumn{1}{l}{Software-Defined Network} \\
    \midrule
    CDN   & Content Delivery Network & GAN   & Generative Adversarial Network & \multicolumn{1}{c}{SGD} & \multicolumn{1}{l}{Stochastic Gradient Descent} \\
    \midrule
    CNN   & Convolutional Neural Network & GNNs  & Graph Neural Networks & \multicolumn{1}{c}{SINR} & \multicolumn{1}{l}{Signal-to-Interference-plus-Noise Ratio} \\
    \midrule
    CV    & Computer Vision & IID   & Independent and Identically Distributed & \multicolumn{1}{c}{SNPE} & \multicolumn{1}{l}{Snapdragon Neural Processing Engine} \\
    \midrule
    D2D   & Device-to-Device & IoT   & Internet of Things & \multicolumn{1}{c}{SRAM} & \multicolumn{1}{l}{Static Random Access Memory} \\
    \midrule
    DDoS  & Distributed Denial of Service & IoV   & Internet of Vehicles & \multicolumn{1}{c}{TL} & \multicolumn{1}{l}{Transfer Learning} \\
    \midrule
    DDPG  & Deep Deterministic Policy Gradient & KD    & Knowledge Distillation & \multicolumn{1}{c}{VM} & \multicolumn{1}{l}{Virtual Machine} \\
    \midrule
    DGC   & Deep Gradient Compression & $k$NN   & $k$-Nearest Neighbor & \multicolumn{1}{c}{VR} & \multicolumn{1}{l}{Virtual Reality} \\
    \midrule
    DL    & Deep Learning & MAB   & Multi-Armed Bandit & \multicolumn{1}{c}{V2V} & \multicolumn{1}{l}{Vehicle-to-Vehicle} \\
    \midrule
    DNNs  & Deep Neural Networks & MDCs  & Micro Data Centers & \multicolumn{1}{c}{WLAN} & \multicolumn{1}{l}{Wireless Local Area Network} \\
    \midrule
    DQL   & Deep Q-Learning & MDP   & Markov Decision Process & \multicolumn{1}{c}{ZB} & \multicolumn{1}{l}{Zettabytes} \\
    \midrule
    DRAM  & Dynamic RAM & MLP   & Multi-Layer Perceptron &       &  \\
    \midrule
    DRL   & Deep Reinforcement Learning & NLP   & Natural Language Processing &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:abbreviation}%
\end{table*}%


==> Tables/TableDLforEdgeV1.tex <==
% 1
% \begin{table*}[tp]  
%     \centering  
%     \fontsize{6.5}{8}\selectfont  
%     \begin{threeparttable}  
%         \caption{Optimization method summary table}  
%         \label{comparison}  
%         \begin{tabular}{p{2.8cm}<{\centering}p{2.4cm}<{\centering}p{1cm}<{\centering}p{2.7cm}<{\centering}p{7.5cm}}  
%             %如果是右对齐，那么只需要将\centering换成\raggedleft，如果左对齐，那么换成\raggedright即可。
%             \toprule  
            
%             \multicolumn{1}{c}{\bf }&\multicolumn{1}{c}{\bf Related Works}&\multicolumn{1}{c}{\bf DNNs or DRL}&\multicolumn{1}{c}{\bf Related Algorithms and Models}&\multicolumn{1}{c}{\bf Objective}\cr
%             \midrule  
            
%             \multirow{8}{*}{Adaptive Edge Caching Policy}&  
%             L. Lei \textit{et al.}\cite{8108157}&DL&AE \& FCNN&Reduce the complexity of conventional optimization algorithms.\cr
%             &Z. Chang \textit{et al.}\cite{Chang2018a}&DL&FCNN& Estimate content popularity and deduce proactive caching strategy.\cr
%             &J. Yang \textit{et al.}\cite{Yang2019b}&DL&CNN&Avoid the repeated calculation of cache refreshing optimization.\cr
%             &A. Ndikumana \textit{et al.}\cite{Ndikumana2018}&DL&FCNN&Train caching policies in the self-driving car to minimize content downloading delay.\cr
%             &Y. Tang \textit{et al.}\cite{Tang2019}&DL&RNN&Predict user mobility and cache contents of users interest in advance.\cr
%             &Y. Wei \textit{et al.}\cite{Wei2018} & DRL & AC & Schedule users and content caching to minimize the average transmission delay. \cr
%             &C. Zhong \textit{et al.}\cite{Zhong2018}&DRL&DDPG& Maximize the long-term cache hit rate.\cr            
%             \cmidrule(lr){1-5}	
            
%             \multirow{10}{*}{Task Offloading Optimization}&  
%             S. Yu \textit{et al.}\cite{Yu2018b}&DL&FCNN& Optimize offloading actions to minimize the computation and offloading overhead.\cr
%             &N. C. Luong \textit{et al.}\cite{Luong2018a}& DL & FCNN & Develop an optimal auction based on DL for the edge resource allocation.\cr
%             &T. Yang \textit{et al.}\cite{Yang2018c}&DRL&DQL&Allocate computational resource for offloaded tasks in order to improve the average end-to-end reliability.\cr
%             &Q. Zhang \textit{et al.}\cite{Zhang2018g}&DRL&Double-DQL&Adaptively select dynamic voltage and frequency scaling algorithms for energy-efficient edge scheduling.\cr
%             &J. Li \textit{et al.}\cite{Li2018h}&DRL&DQL& Determine the computation offloading decision and the allocated computation resource of all edge devices.\cr
%             &Z. Chen \textit{et al.}\cite{Chenc}&DRL&DDPG&Perform more fine-grained power control for local execution and task offloading.\cr
%             &M. Min \textit{et al.}\cite{Min2017}&DRL&DQL&Choose the MEC server and determine the offloading rate in energy harvesting environment.\cr
%             &X. Chen \textit{et al.}\cite{Chen2018k}&DRL&Double-DQL&Optimize computation offloading policies for a virtual MEC system.\cr
%             &L. Huang \textit{et al.}\cite{Huang}&DRL&FCNN&Reduce the computational complexity without compromising the solution quality.\cr
            
%             \cmidrule(lr){1-5}	
%             \multirow{7}{*}{Intelligent Edge Management}& 
%             S. Memon \textit{et al.}\cite{Memon2018}&DL&RNN \& LSTM &Assist the smooth transition of device connections and offloaded tasks between edge nodes.\cr
%             &Y. Sun \textit{et al.}\cite{Sun2018a}&DRL&DQL \& TL &Control communication modes of edge devices and on-off states of their processors to minimize long-term system power consumption.\cr
%             \cmidrule(lr){2-5}
%             &L. Xiao \textit{et al.}\cite{Xiao2018a}&DRL&DQL&Provide secure offloading from the edge device to the edge node against jamming attacks.\cr
%             \cmidrule(lr){2-5}
%             &Y. He \textit{et al.}\cite{He2017a}&DRL&DQL&Improve the servicing performance of the edge computing network.\cr
%             &Y. Wei \textit{et al.}\cite{Wei2018b}&DRL&AC&Minimizing the average end-to-end servicing delay.\cr
%             &Y. He \textit{et al.}\cite{He2018e}&DRL&Double-Dueling DQL&Improve the performance of future IoVs.\cr
%             &L. T. Tan \textit{et al.}\cite{Le2018a}&DRL&DQL&Optimize caching placement and computing resource allocation as well as to determine possible connecting RSUs and neighboring vehicles.\cr

%             \bottomrule  
%         \end{tabular}  
%     \end{threeparttable}  
% \end{table*}

% 2
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp!!!!]
%     \centering
%     \scriptsize
%     % \fontsize{6.5}{8}\selectfont  
%     \caption{DL for Optimizing Edge Application Scenarios}
%     \label{tab:DLforEdge}%
%       \begin{tabular}{cccccl}
%       \toprule
%             &       & \multicolumn{1}{c}{\textbf{\tabincell{c}{Related \\ Work}}} & \textbf{\tabincell{c}{DNNs \\ or \\ DRL}} & \textbf{\tabincell{c}{Related \\ Methods}} & \multicolumn{1}{c}{\textbf{Objective}} \\
%       \midrule
%       \multicolumn{2}{c}{\multirow{9}[14]{*}{\textbf{\tabincell{c}{Adaptive \\ Edge \\ Caching \\ Policy}}}} &    \multicolumn{1}{c}{\cite{8108157}}   & DL    & AE \& FCNN & Reduce the complexity of conventional optimization algorithms \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Chang2018a}}   & DL    & FCNN  & Estimate content popularity and deduce proactive caching strategies \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Yang2019b}}    & DL    & CNN   & Avoid the repeated calculation of cache refreshing optimization \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Ndikumana2018}}    & DL    & FCNN  & \multicolumn{1}{l}{\tabincell{l}{Train caching policies in the self-driving car to \\ minimize content downloading delay}} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Tang2019}}   & DL    & RNN   & \tabincell{l}{Predict user mobility and cache contents \\ of users interest in advance} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Wei2018}}   & DRL   & AC    & \tabincell{l}{Schedule users and content caching \\ to minimize the average transmission delay} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Zhong2018}}    & DRL   & DDPG  & Maximize the long-term cache hit rate \\
%       \midrule
%       \multicolumn{2}{c}{\multirow{15}[18]{*}{\textbf{\tabincell{c}{Task \\ Offloading \\ Optimization}}}} &    \multicolumn{1}{c}{\cite{Yu2018b}}   & DL    & FCNN  & \tabincell{l}{Optimize offloading actions to \\ minimize the computation and offloading overhead} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Luong2018a}}   & DL    & FCNN  & \tabincell{l}{Develop an optimal auction based on DL \\ for the edge resource allocation} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Yang2018c}}    & DRL   & DQL   & \tabincell{l}{Allocate computational resource for offloaded  \\ tasks in order to improve the average end-to-end reliability} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Zhang2018g}}    & DRL   & Double-DQL  & \tabincell{l}{Adaptively select dynamic voltage and frequency \\ scaling algorithms for energy-efficient edge scheduling} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Li2018h}}    & DRL   & DQL   & \tabincell{l}{Determine the computation offloading decision and \\ the allocated computation resource of all edge devices} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &  \multicolumn{1}{c}{\cite{Chenc}}     & DRL   & DDPG  & \tabincell{l}{Perform more fine-grained power control \\ for local execution and task offloading} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Min2017}}   & DRL   & DQL   & \tabincell{l}{Choose the MEC server and determine the offloading rate \\ in energy harvesting environment} \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Chen2018k}}    & DRL   & Double-DQL & Optimize computation offloading policies for a virtual MEC system \\
%   \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Huang}}    & DRL   & FCNN  & \tabincell{l}{Reduce the computational complexity \\ without compromising the solution quality} \\
%       \midrule
%       \multicolumn{1}{c}{\multirow{11}[14]{*}{\textbf{\tabincell{c}{ Edge \\ Management \\ and \\ Maintenance}}}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{\tabincell{c}{Edge \\ Communication}}}} &    \multicolumn{1}{c}{\cite{Memon2018}}   & DL    & RNN \& LSTM  & \tabincell{l}{Assist the smooth transition of device connections \\ and offloaded tasks between edge nodes} \\
%   \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Sun2018a}}    & DRL   & DQL \& TL  & \tabincell{l}{Control communication modes of edge devices and on-off states \\ of their processors to minimize long-term system power consumption} \\
%   \cmidrule{2-6}          & \multicolumn{1}{c}{\textbf{\tabincell{c}{Edge \\ Security}}} &  \multicolumn{1}{c}{\cite{Xiao2018a}}     & DRL   & DQL   & \tabincell{l}{Provide secure offloading from the edge device \\ to the edge node against jamming attacks} \\
%   \cmidrule{2-6}          & \multicolumn{1}{c}{\multirow{5}[8]{*}{\textbf{\tabincell{c}{Joint \\ Edge \\ Optimization}}}} &    \multicolumn{1}{c}{\cite{He2017a}}   & DRL   & DQL   & Improve the servicing performance of the edge computing network \\
%   \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Wei2018b}}    & DRL   & AC    & Minimize the average end-to-end servicing delay \\
%   \cmidrule{3-6}          &       &    \multicolumn{1}{c}{\cite{He2018e}}   & DRL   & \tabincell{c}{Double-Dueling \\ DQL}  & Improve the performance of future IoVs \\
%   \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Le2018a}}    & DRL   & DQL   & \tabincell{l}{Optimize caching placement and computing resource allocation \\ as well as to determine possible connections} \\
%       \bottomrule
%       \end{tabular}%
% \end{table*}%
  
\begin{table*}[htbp!!!!]
    \centering
    \scriptsize
    % \fontsize{6.5}{8}\selectfont  
    \caption{DL for Optimizing Edge Application Scenarios}
    \label{tab:DLforEdge}%
      \begin{tabular}{cccccl}
      \toprule
            &       & \multicolumn{1}{c}{\textbf{\tabincell{c}{Related \\ Work}}} & \textbf{\tabincell{c}{DNNs \\ or \\ DRL}} & \textbf{\tabincell{c}{Related \\ Methods}} & \multicolumn{1}{c}{\textbf{Objective}} \\
      \midrule
      \multicolumn{2}{c}{\multirow{7}[14]{*}{\textbf{\tabincell{c}{Adaptive \\ Edge \\ Caching \\ Policy}}}} &      \multicolumn{1}{c}{\cite{Chang2018a}}   & DL    & FCNN  & Estimate content popularity and deduce proactive caching strategies \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Yang2019b}}    & DL    & CNN   & Avoid the repeated calculation of cache refreshing optimization \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Ndikumana2018}}    & DL    & FCNN  & \multicolumn{1}{l}{\tabincell{l}{Train caching policies in the self-driving car to \\ minimize content downloading delay}} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Tang2019}}   & DL    & RNN   & \tabincell{l}{Predict user mobility and cache contents \\ of users interest in advance} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Wei2018b}}   & DRL   & AC    & \tabincell{l}{Schedule users and content caching \\ to minimize the average transmission delay} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Zhong2018}}    & DRL   & DDPG  & Maximize the long-term cache hit rate \\
      \midrule
      \multicolumn{2}{c}{\multirow{15}[18]{*}{\textbf{\tabincell{c}{Task \\ Offloading \\ Optimization}}}} &    \multicolumn{1}{c}{\cite{Yu2018b}}   & DL    & FCNN  & \tabincell{l}{Optimize offloading actions to \\ minimize the computation and offloading overhead} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Luong2018a}}   & DL    & FCNN  & \tabincell{l}{Develop an optimal auction based on DL \\ for the edge resource allocation} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Yang2018c}}    & DRL   & DQL   & \tabincell{l}{Allocate computational resource for offloaded  \\ tasks in order to improve the average end-to-end reliability} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Zhang2018g}}    & DRL   & Double-DQL  & \tabincell{l}{Adaptively select dynamic voltage and frequency \\ scaling algorithms for energy-efficient edge scheduling} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Li2018h}}    & DRL   & DQL   & \tabincell{l}{Determine the computation offloading decision and \\ the allocated computation resource of all edge devices} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &  \multicolumn{1}{c}{\cite{Chenc}}     & DRL   & DDPG  & \tabincell{l}{Perform more fine-grained power control \\ for local execution and task offloading} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &    \multicolumn{1}{c}{\cite{Min2017}}   & DRL   & DQL   & \tabincell{l}{Choose the MEC server and determine the offloading rate \\ in energy harvesting environment} \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Chen2018k}}    & DRL   & Double-DQL & Optimize computation offloading policies for a virtual MEC system \\
  \cmidrule{3-6}    \multicolumn{2}{c}{} &   \multicolumn{1}{c}{\cite{Huang}}    & DRL   & FCNN  & \tabincell{l}{Reduce the computational complexity \\ without compromising the solution quality} \\
      \midrule
      \multicolumn{1}{c}{\multirow{11}[14]{*}{\textbf{\tabincell{c}{ Edge \\ Management \\ and \\ Maintenance}}}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{\tabincell{c}{Edge \\ Communication}}}} &    \multicolumn{1}{c}{\cite{Memon2018}}   & DL    & RNN \& LSTM  & \tabincell{l}{Assist the smooth transition of device connections \\ and offloaded tasks between edge nodes} \\
  \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Sun2019}}    & DRL   & DQL \& TL  & \tabincell{l}{Control communication modes of edge devices and on-off states \\ of their processors to minimize long-term system power consumption} \\
  \cmidrule{2-6}          & \multicolumn{1}{c}{\textbf{\tabincell{c}{Edge \\ Security}}} &  \multicolumn{1}{c}{\cite{Xiao2018a}}     & DRL   & DQL   & \tabincell{l}{Provide secure offloading from the edge device \\ to the edge node against jamming attacks} \\
  \cmidrule{2-6}          & \multicolumn{1}{c}{\multirow{5}[8]{*}{\textbf{\tabincell{c}{Joint \\ Edge \\ Optimization}}}} &    \multicolumn{1}{c}{\cite{He2017a}}   & DRL   & DQL   & Improve the servicing performance of the edge computing network \\
  \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Wei2018b}}    & DRL   & AC    & Minimize the average end-to-end servicing delay \\
  \cmidrule{3-6}          &       &    \multicolumn{1}{c}{\cite{He2018e}}   & DRL   & \tabincell{c}{Double-Dueling \\ DQL}  & Improve the performance of future IoVs \\
  \cmidrule{3-6}          &       &   \multicolumn{1}{c}{\cite{Le2018a}}    & DRL   & DQL   & \tabincell{l}{Optimize caching placement and computing resource allocation \\ as well as to determine possible connections} \\
      \bottomrule
      \end{tabular}%
\end{table*}%

==> Tables/TableDLinEdgeChallgenge.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp!!!!!!!!!]
  \centering
  \scriptsize
  \caption{Research Directions and Challenges of ``DL in Edge''}
    \begin{tabular}{llll}
    \toprule
    \multicolumn{1}{c}{\textbf{Research Direction}} & \multicolumn{1}{c}{\textbf{Existing Limitation}} & \multicolumn{1}{c}{\textbf{\tabincell{c}{Challenge or \\ Potential Solution} }} & \multicolumn{1}{c}{\textbf{Metric}} \\
    \midrule
    \tabincell{l}{Generalization \\ of EEoI} & \tabincell{l}{EEoI can only be applied \\ to classification problems.} &  EEoI for DRL     & \textbullet~Extensive application \\
    \midrule
    \tabincell{l}{Hybrid model \\ modification} & \tabincell{l}{Efficent combination is missing \\ between model optimization, \\ segmentation and EEoI.} &  \tabincell{l}{Hybrid precision \\scheme} &  \tabincell{l}{\textbullet~Overhead \\ \textbullet~Inference latency \\ \textbullet~Model accuracy} \\
    \midrule
    \tabincell{l}{Coordination between \\ training and inference} & \tabincell{l}{Continuous online DL training \\ affects DL inference in the edge.} &  \tabincell{l}{Balance mechanism} &  \tabincell{l}{\textbullet~Overhead \textbullet~Training speed \\ \textbullet~Inference latency \textbullet~Model accuracy} \\
    \bottomrule
    \end{tabular}%
  \label{tab:DLinEdgeChallgenge}%
\end{table*}%

==> Tables/TableEdgeforDLChallgenge.tex <==
\begin{table*}[htbp!!!!!!!!!!]
  \centering
  \scriptsize
  \caption{Research Directions and Challenges of ``Edge for DL''}
    \begin{tabular}{llll}
    \toprule
    \multicolumn{1}{c}{\textbf{\tabincell{c}{Research \\ Direction}}} & \multicolumn{1}{c}{\textbf{Expected Objective}} & \multicolumn{1}{c}{\textbf{\tabincell{c}{Challenge or \\ Potential Solution}}} & \multicolumn{1}{c}{\textbf{Metric}} \\
    \midrule
    \tabincell{l}{Edge for \\ data processing} & \multicolumn{1}{l}{\tabincell{l}{\textbullet~Efficiently acquire and process \\ ~~massive sensed or collected data \\ ~~by edge infrastructures}} & \tabincell{l}{\textbullet~Adaptive data acquirement \\ \textbullet ~Adaptive data compression \\ \textbullet~Universal or customized architecture} & \tabincell{l}{\textbullet~Overhead, \\ \textbullet~Processing speed, \\ \textbullet~Throughput} \\
    \midrule
    \tabincell{l}{Reduction of \\ DL computation} & \multicolumn{1}{l}{\tabincell{l}{\textbullet~Dispose DL requests at the edge \\ ~~without redundant computation}} & \tabincell{l}{\textbullet~DRL support \textbullet~Cache inference results \\ \textbullet~Deploy multiple DL models \\ \textbullet~Sharing intermediate DL inference results} & \tabincell{l}{\textbullet~Overhead, \\ \textbullet~Inference latency, \\\textbullet~Model accuracy} \\
    \midrule
    \tabincell{l}{Microservice \\ for DL services} & \multicolumn{1}{l}{\tabincell{l}{\textbullet~Host DL services on microservice \\ ~~frameworks deployed on the edge}} & \tabincell{l}{\textbullet~Microservice framework for edge computing \\ \textbullet~Live migration of microservices \\ \textbullet~Coordination between the cloud and the edge} & \tabincell{l}{\textbullet~Overhead,\\ \textbullet~Throughput,\\ \textbullet~Stability} \\
    \midrule
    \tabincell{l}{Incentive and \\ trusty offloading} & \tabincell{l}{\textbullet~Provide edge nodes with incentives \\ ~~to take over DL computations \\ \textbullet~Guarantee the security to avoid the \\ ~~risks from anonymous edge nodes}  & \tabincell{l}{\textbullet~Apply blockchain in the edge architecture \\ \textbullet~Existing blockchain solutions do not \\ ~~support the execution of DL} & \tabincell{l}{\textbullet~Overhead, \\\textbullet~Throughput,\\ \textbullet~Security, \\\textbullet~Inference latency} \\
    \midrule
    \tabincell{l}{Edge architecture \\ and testbed for DL} & \tabincell{l}{\textbullet~Automate phases of the DL \\ ~~development process \\ \textbullet~Practically supporting ideas \\ ~~in Section \ref{subsec:edgecomputingmodefordl} \\ \textbullet~Testify and optimize the performance \\ ~~of DL services on the edge} & \tabincell{l}{\textbullet~Exploit underlying edge hardware \\ ~~in terms of performance and power \\ \textbullet~Develop a standard and comprehensive \\ ~~testbed} & \tabincell{l}{\textbullet~Overhead, \\ \textbullet~Inference latency,\\ \textbullet~Throughput, \\ \textbullet~Stability} \\
    \bottomrule
    \end{tabular}%
  \label{tab:EdgeforDLChallgenge}%
\end{table*}%

==> Tables/TableModelOptimization.tex <==
% \begin{table*}[tp]  
%     \centering  
%     \fontsize{6.5}{8}\selectfont  
%     \begin{threeparttable}  
%         \caption{Optimization methods of DL models in edge}  
%         \label{optimization_summary}  
%         \begin{tabular}{cllll}  
%             \toprule  
%             \multicolumn{1}{c}{\bf Classification}&\multicolumn{2}{c}{\bf Optimization}&\multicolumn{1}{c}{\bf Classification}\cr
%             \midrule  
%             \specialrule{0em}{3pt}{1pt}
%             \cmidrule(lr){1-3}
%             \specialrule{0em}{1pt}{1pt}
%             \cmidrule(lr){2-4}
%             \multirow{4}{*}{General Model Optimization Methods}&\multicolumn{2}{l}{Parameter pruning and sharing\cite{Han2015, Alwani2016,Han2017, Mao2016b, Bhattacharya,Shen2014}}&\multirow{12}{*}{Model optimization for edge devices} \cr
%             &\multicolumn{2}{l}{Low-rank factorization\cite{Denton2014}}& \cr
%             &\multicolumn{2}{l}{Transferred/Compact convolution filters\cite{Iandola2017, Howard2012, Nikouei2018a}}& \cr
%             &\multicolumn{2}{l}{Knowledge distillation\cite{Sharma2018,Yao2017}}& \cr
%             \cmidrule(lr){1-3}
%             &Narrowing down the classifier’s searching space\cite{Nikouei2018}&Model inputs optimization& \cr
%             \cmidrule(lr){2-3}
%             &Modifies convolution operations\cite{Zhang,Du2018,c}&\multirow{2}{*}{Model structures optimization}& \cr
%             &Design a hardware architecture\cite{Han2017}& \cr
            
%             \cmidrule(lr){2-3}
%             &Provides a library of optimized software kernels\cite{Lai2018}&\multirow{5}{*}{Model frameworks optimization}& \cr
%             &Automatically compresses DL models\cite{Yao2017}& \cr
%             &Performs quantization and coding on all commonly used DL structures\cite{Mao2016b, Shen2014, Yao2017}& \cr
%             &Specializes DL models to contexts\cite{Shen2014}& \cr 
%             &Fitted in on-chip SRAM\cite{Han2016}& \cr 
%             \cmidrule(lr){2-4}	

            
%             \bottomrule  
%         \end{tabular}  
%     \end{threeparttable}  
% \end{table*}

\begin{table*}
    \centering
    \caption{Optimization methods of DL models in edge}
    \label{optimization_summary}
    \begin{tabular}{clll} 
    \toprule
     & \multicolumn{2}{c}{\textbf{Optimization}} & \multicolumn{1}{c}{} \\ 
    \midrule
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}General model \\optimization methods\end{tabular}} & \multicolumn{2}{l}{Parameter pruning and sharing} & \multirow{12}{*}{\begin{tabular}[c]{@{}l@{}}Model optimization\\~for edge devices\end{tabular}} \\
     & \multicolumn{2}{l}{Low-rank factorization} &  \\
     & \multicolumn{2}{l}{Transferred/Compact convolution filters} &  \\
     & \multicolumn{2}{l}{Knowledge distillation} &  \\ 
    \cmidrule{1-3}
     & Narrowing down the classifier’s searching space & Model inputs optimization &  \\ 
    \cmidrule{2-3}
     & Modifies convolution operations & \multirow{2}{*}{Model structures optimization} &  \\
     & Design a hardware architecture &  &  \\ 
    \cmidrule{2-3}
     & Provides a library of optimized software kernels & \multirow{5}{*}{Model frameworks optimization} &  \\
     & Automatically compresses DL models &  &  \\
     & Performs quantization and coding on all commonly used DL structures &  &  \\
     & Specializes DL models to contexts &  &  \\
     & Fitted in on-chip SRAM &  &  \\
    \bottomrule
    \end{tabular}
\end{table*}
